Determinantal Facet Ideals for Smaller Minors

A determinantal facet ideal (DFI) is generated by a subset of the maximal minors of a generic $n\times m$ matrix where $n\leq m$ indexed by the facets of a simplicial complex $\Delta$. We consider the more general notion of an $r$-DFI, which is generated by a subset of $r$-minors of a generic matrix indexed by the facets of $\Delta$ for some $1\leq r\leq n$. We define and study so-called lcm-closed and unit interval $r$-DFIs, and show that the minors parametrized by the facets of $\Delta$ form a reduced Gr\"obner basis with respect to \emph{any} term order for an lcm-closed $r$-DFI. We also see that being lcm-closed generalizes conditions previously introduced in the literature, and conjecture that in the case $r=n$, lcm-closedness is necessary for being a Gr\"obner basis. We also give conditions on the maximal cliques of $\Delta$ ensuring that lcm-closed and unit interval $r$-DFIs are Cohen-Macaulay. Finally, we conclude with a variant of a conjecture of Ene, Herzog, and Hibi on the Betti numbers of certain types of $r$-DFIs, and provide a proof of this conjecture for Cohen-Macaulay unit interval DFIs.

==> revisionLetter.tex <==
Revision Letter for ``Determinantal Facet Ideals for Smaller Minors''

Thank you very much for your feedback. Based on the referee's commments, we have implemented some changes to improve the readability and clarity of the article based on comments 1-6.

We would like to directly address comment 7 by the referee. Note that $r$ is fixed in Definition 2.11, so all generators of $J_\Delta$ correspond to $r\times r$ minors of a generic matrix. In particular, any generators coming from $J_{\Delta_i}\cap J_{\Delta_j}$ correspond to $(r-1)$-dimensional faces of $J_{\Delta_i}\cap J_{\Delta_j}$, which in turn are $(r-1)$-dimensional faces of $J_{\Delta_i}$ and $J_{\Delta_j}$, which themselves are $(r-1)$-dimensional faces of $J_\Delta$. To clarify our notation and definitions further, we have added Example 2.12.

We made one other significant change: we have been informed by Bruno Benedetti and Matteo Varbaro that the phrase ``interval DFI'' clashes with the notion of an ``interval graph'' in combinatorics. In the case when $G$ is a graph, our notion of ``interval DFI'' actually corresponds to the case of ``unit interval graphs''. For this reason, we have chosen to rename interval DFIs to ``unit interval DFIs'' for clarity.


==> revisionletter2.tex <==
Thank you very much for your feedback. We address each of the referee's individual comments below.

\begin{enumerate}[(1)]
\item The definition of a clique decomposition does not depend on $\Delta$ being pure. We require that $\Delta$ be pure in later definitions for the reasons you state. We have added this hypothesis to Definition 2.3.
\item In this definition, we refer the reader specifically to Notation 2.1, which establishes exactly what the hypotheses on $\aa$ and $\bb$ are.
\item The intersection of two simplices is a simplex on the vertices contained in both simplices. Indeed, as you suggest, if the dimension of the intersection is ``too small'', then any minor $[\aa\mid\bb]\in J_{\Delta_i}$ must have a leading term which is coprime to that of any minor $[\aa'\mid \bb']\in J_{\Delta_j}$ in order for the simplicial complex to be considered ``lcm-closed''. This is exactly what happens in Example 2.14.
\item The term order is noted in Notation 2.8. We have now added a direct reference to Notation 2.8 for the ease of the reader.
\item We have now added a direct reference to Definition 2.10 for the ease of the reader. We established our conventions in Notation 2.1 for the conditions on $\aa$ and $\bb$, but we have now also added a direct reference to Notation 2.1 for the ease of the reader.
\item Thank you for pointing out this typo. We have corrected $[\aa]$ and $[\bb]$ to $\inn[\aa]$ and $\inn[\bb]$.
\end{enumerate}

==> revisionletter3.tex <==
We think that we understand the confusion for DFIs: implicit in most papers written on DFIs in the understanding that a DFI is totally determined by the $(r-1)$-skeleton of the associated simplicial complex. That is, it is not even relevant that the parametrizing simplicial complex be $(r-1)$-dimensional nor pure, since one only cares about faces inducing column sets of the correct size. If a simplicial complex has dimension strictly smaller than $r-1$ (and one specifies that they only care about $r$-minors, which is why we write $r$-DFI), then the $r$-DFI corresponding to this simplicial complex is the $0$ ideal (that is, it is generated by the empty set). 

It is unfortunate that the pre-existing literature on DFIs has used the terminology of simplicial complexes, since it is actually totally unnecessary. More precisely, one can instead define an $r$-DFI as induced by a subset $S$ of $P_r ([n])$ (this notation means all subsets of $[m]$ with size $r$); in this case, ``maximal cliques" are just the largest subsets $T$ of $[m]$ from which all $r$-subsets of $T$ are contained in $S$. Since intersections of subsets of $P_r ([m])$ are still subsets of $P_r ([m])$, the concerns about maximal clique intersections are no longer an issue. We have decided not to reformulate the paper with this language, again because the pre-existing literature has made the notation we currently use standard. However, we thought it would be useful to include this reformulation since we unconsciously tend to associate the simplicial complex $\Delta$ with its faces of dimension $r-1$ (and ignore the rest).

We have updated the paper is accordance with the comments of the referee (hopefully these changes are not viewed as superficial this time; we did not intend them to seem that way in earlier drafts, and apologize for that).

\begin{enumerate}
    \item For your comment $(1)$: we have deleted the assumption ``pure" in the definition of an $r$-DFI and specified that it is only the $(r-1)$-faces of $\Delta$ that have any effect on the $r$-DFI $J_\Delta$. However, we have kept the ``pure" assumption whenever we impose the maximal clique decomposition; this is sufficient for $r$-DFIs in full generality since one may replace an arbitrary simplicial complex $\Delta$ with the simplicial complex whose facets are simply the $(r-1)$-faces of $\Delta$. This will induce the same $r$-DFI and be pure by construction. At no point in the paper do we utilize a clique decomposition for intersections of maximal cliques $\Delta_i \cap \Delta_j$, so this does not conflict with proofs as currently written.
    \item This remark has been re-written; it is not true that an arbitrary collection of minors corresponds to an $r$-DFI with our definition. The main point of this remark was to attempt to give an abridged version of the beginning of this report.
    \item Hopefully the discussion at the beginning of this report has clarified this. Just to be clear: if $\Delta$ is not pure, the definition of $r$-DFI still makes sense. If the set of $(r-1)$-dimensional faces of $\Delta$ is empty, then the associated $r$-DFI is the $0$ ideal. 
    \item This was a typo, it is not relevant that $<$ be the standard diagonal term order; we only care that the initial term of each minor is the product of the diagonals (actually, as formulated now, the definition of lcm-closed no longer depends on the term order).
    \item You are correct (this definition was originally written in another paper only for maximal minors, so this is why the indices were assumed equal). So as to be more clear (and remove the dependence on the term order), we have simply replaced this condition with ``with non-coprime lead terms"; hopefully this clear up the confusion.
\end{enumerate}

==> revisionletter4.tex <==
In an earlier version of the paper, we generalized our definition of lcm-closed to allow for arbitrary term orders (rather than only the standard diagonal term order). In this version we have adjusted the statements of several results throughout our paper to reflect that they hold in this level of generality. We also added a proof that in the case when $n=2$, Question 2.18 has a positive answer (see Proposition 2.19).

Thank you very much for catching the mistake in our proof of Proposition 2.17. In the process of correcting this mistake, we were forced to add more cases which led to a long and computationally intense proof with many lemmas and identities we were required to prove along the way. This proof would have taken us far over the recommended page limit for ADM, so we decided instead to cite a result of Lisa Seccia for the proof, since she proved a more general result independently with more elegant methods. 

==> sections/LinStrand.tex <==
\section{Linear Strand of the Initial Ideal of Certain Determinantal Facet Ideals}\label{sec:linearstrandofintl}

In this section, we consider certain more general classes of determinantal facet ideals whose minimal generating set may \emph{not} form a Gr\"obner basis.
We introduce the idea of an $i$-nonface, which can be used to measure the homology of a complex introduced in Definition \ref{def:gensparseEN}.
For a simplicial complex with no $1$-nonfaces of cardinality $n+1$, we prove that this \emph{generalized} sparse Eagon-Northcott complex is isomorphic to the linear strand of the initial ideal (with respect to the standard diagonal term order) of the associated $n$-determinantal facet ideal.
% We then consider the case where the minimal generating set of the associated determinantal facet ideal \emph{does} form a Gr\"obner basis.
% In this case, we can use Corollary \ref{cor: linearStrandDFI} to independently prove that the linear strand is isomorphic to the complex of Definition \ref{def:gensparseEN}.
% As an immediate consequence, this gives a necessary combinatorial condition for the minimal generators of a determinantal facet ideal to form a Gr\"obner basis (see Corollary \keller{Cite once cor is written}). 

\begin{setup}\label{set:linearStrandSetup}
Let $R= k[x_{ij} \mid 1\leq i \leq n, 1 \leq j \leq m]$ and $M = (x_{ij})_{1\leq i \leq n, 1 \leq j \leq m}$ denote a generic $n \times m$ matrix, where $n \leq m$. View $M$ as a homomorphism $M : F \to G$ of free modules $F$ and $G$ of rank $m$ and $n$, respectively.

Let $f_i$, $i=1, \dots , m$, $g_j$, $j=1 , \dots , n$ denote the standard bases with respect to which $M$ has the above matrix representation. Let $<$ denote standard lexicographic order on $R$ and $\inn_< I_n(M)$ the initial ideal with respect to $<$ of the ideal of maximal minors of $M$.
\end{setup}

\begin{notation}
Let $\alpha = (\alpha_1 , \dotsc , \alpha_n)$. Define
$$\alpha_{\leq i } := (\alpha_1 , \dotsc , \alpha_i ),$$
where $\alpha_{\leq i} = \varnothing$ if $i \leq 0$ and $\alpha_{\leq i } = \alpha$ if $i \geq n$.
\end{notation}

\begin{definition}\label{def:sparseENdiff}
Let $\alpha = (\alpha_1 , \dotsc , \alpha_n)$ with $|\alpha | = \ell$ and $I = (i_1 < \cdots < i_{n+\ell})$. Define the indexing set
$$\I_< ( \alpha , I) := \{ (i , I_{i+j}) \mid i \in \{ k \mid \alpha_k >0 \}, \ |\alpha_{\leq i-1}| \leq j \leq |\alpha_{\leq i}| \}$$
\end{definition}

\begin{example}
One easily computes:
$$\I_< ( (1,1,1) , (1,2,3,4,5,6) ) = \{(1,1), (1,2), (2,3), (2,4), (3,5), (3,6)\}$$
$$\I_< ( (1,0,2),(1,2,3,4,5,6)) = \{(1, 1), (1, 2), (3, 4), (3, 5), (3, 6)\}$$
$$\I_< ((2,1),(1,2,4,5,6)) = \{(1, 1), (1, 2), (1, 4), (2, 5), (2, 6)\}$$
\end{example}

\begin{theorem}[\cite{herzog2015linear}, Theorem 1.1]\label{thm:linstrandequiv}
Let $R$ be a standard graded polynomial ring over a field $k$. Let $G_\bullet$ be a finite linear complex of free $R$-modules with initial degree $n$. Then the following are equivalent:
\begin{enumerate}
    \item The complex $G_\bullet$ is the linear strand of a finitely generated $R$-module with initial degree $n$.
    \item The homology $H_i (G_\bullet)_{i+n+j} = 0$ for all $i>0$ and $j=0, \ 1$.
\end{enumerate}
\end{theorem}

\begin{prop}[\cite{herzog2015linear}, Corollary 1.2]\label{prop:linstrandcor}
Let $R$ be a standard graded polynomial ring over a field $k$. Let $G_\bullet$ be a finite linear complex of free $R$-modules with initial degree $n$ such that $H_i (G_\bullet)_{i+n+j} = 0$ for all $i>0$, $j=0, \ 1$. 

Let $N$ be a finitely generated $R$-module with minimal graded free resolution $F_\bullet$. Assume that there exist isomorphisms making the following diagram commute:
$$\xymatrix{G_1 \ar[d]_-{\sim} \ar[r] & G_0 \ar[d]^-{\sim} \\
F_1^{\textrm{lin}} \ar[r] & F_0^{\textrm{lin}}. \\}$$
Then $G_\bullet \cong F_\bullet^\textrm{lin}$.
\end{prop}

\begin{definition}\label{def:gensparseEN}
Adopt notation and hypotheses as in Setup \ref{set:linearStrandSetup}. Let $\Delta$ denote a simplicial complex on the vertex set $[m]$. Define $\cat{C}^<_0 (\Delta , M) := \bigwedge^n G$. For $i \geq 1$, let $\cat{C}^<_i (\Delta , M) \subseteq D_{i-1} (G^*) \otimes \bigwedge^{n+i-1} F$ denote the free submodule generated by all elements of the form
$$g^{* ( \alpha)} \otimes f_\sigma,$$
where $\sigma \in \Delta$ with $|\sigma|=n+i-1$ and $\alpha = (\alpha_1 , \dotsc , \alpha_n)$ with $|\alpha| = i-1$. 

Let $\cat{C}^<_\bullet (\Delta , M)$ denote the complex induced by the differential $$d'_1 : \bigwedge^n F \to \bigwedge^n G$$ sending $f_I \mapsto \inn_<  (M(f_I))$ and for $\ell\geq 2$, 
$$d'_\ell : D_{\ell - 1} (G^*) \otimes \bigwedge^{n+\ell-1} F \to D_{\ell-2} (G^*) \otimes \bigwedge^{n+\ell-2} F$$ is the sparse Eagon-Northcott differential
$$d_\ell ( g^{*(\alpha)} \otimes f_I ) = \sum_{\{i \mid \alpha_i >0\}} \sum_{(i,I_j) \in \I_< (\alpha , I)} (-1)^{j + 1}  x_{iI_j} g^{*(\alpha - \epsilon_i)} \otimes f_{I \backslash I_j }.$$
\end{definition}

\begin{definition}\label{def:inonface}
Let $\Delta$ be a simplicial complex. Then an $i$-nonface $\sigma = \{\sigma_1 < \dots < \sigma_\ell\}$ is an element $\sigma \notin \Delta$ such that for some $j\geq 1$, $\sigma \backslash \sigma_{j+k} \in \Delta$ for all $k= 0 , \dotsc , i$. 
\end{definition}

\begin{example}\label{ex:exampleof1nonface}
Consider the following graph $G$ on vertices $\{1,2,3,4 \}$:
$$\xymatrix{3 \ar@{-}[d] & 2 \ar@{-}[dl] \\
4  & 1. \ar@{-}[l] \ar@{-}[ul] \ar@{-}[u] \\}$$
Observe that the associated clique complex has facets $\{1,2,4 \}$ and $\{1,3,4 \}$, and no minimal nonfaces. However, $\{ 1,2,3,4 \}$ is a $1$-nonface of the clique complex, since $\{1,2,4 \}$ and $\{1,3,4 \}$ are both facets.

If we instead consider the graph
$$\xymatrix{3 \ar@{-}[d] & 2 \ar@{-}[l] \ar@{-}[dl] \\
4  & 1,  \ar@{-}[ul] \ar@{-}[u]  \\}$$
then the clique complex has facets $\{ 1,2,3\}$ and $\{2,3,4 \}$. The set $\{1,2,3,4\}$ is not a $1$-nonface. Likewise, there are no $1$-nonfaces of cardinality $3$. In the graph
$$\xymatrix{3 \ar@{-}[d] & 2 \ar@{-}[l] \ar@{-}[dl] \\
4  & 1, \ar@{-}[l] \ar@{-}[u]  \\}$$
the associated clique complex has facets $\{ 1,2,4\}$ and $\{2,3,4 \}$, and has no $1$-nonfaces of cardinality $4$. However, $\{ 1,3,4 \}$ is a $1$-nonface of cardinality $3$ since $\{ 1,4 \}$ and $\{3,4 \}$ are vertices of $G$.
\end{example}

\begin{remark}
Notice that a minimal nonface $\sigma$ is a $\dim \sigma$-nonface in the above definition. Moreover, any $i$-nonface is a $k$-nonface for all $k \leq i$. 
\end{remark}

In the proofs of the results in the remainder of this section, notice that we have chosen to augment our complexes with the ring $R$. This means that we are resolving the quotient ring $R/I$ as opposed to the module $I$; this has the effect of shifting the indexing in the statements of Theorem \ref{thm:linstrandequiv} and Proposition \ref{prop:linstrandcor}.

\begin{lemma}\label{lem:linstrandnonfaces}
Adopt notation and hypotheses as in Setup \ref{set:linearStrandSetup}. If the simplicial complex $\Delta$ has no $1$-nonfaces of cardinality $\geq n+1$, then the complex $\cat{C}^<_\bullet (\Delta , M)$ is the linear strand of a finitely generated graded $R$-module with initial degree $n$.
\end{lemma}


\begin{proof}
Employ Theorem \ref{thm:linstrandequiv}. To avoid trivialities, assume $n \leq \dim (\Delta) + 1$. Observe first that $H_i (\cat{C}_\bullet^< ( \Delta , M))_{i+n-1} = 0$ for all $i \geq 1$ trivially.

To finish the proof, we show that
$$H_i (\cat{C}_\bullet^< ( \Delta , M))_{i+n} \neq 0 \ \textrm{for all} \ i \geq 1$$
$$\implies$$
$$\textrm{there exists a} \ 1\textrm{-nonface of cardinality} \ n+i, \ \textrm{for all} \ i\geq 1.$$
For convenience, use the notation $\cat{C}_\bullet^< (M) =: E_\bullet'$, where $\cat{C}_\bullet^< (M)$ is as in Definition \ref{def:gensparseEN}. 

Assume $H_i (\cat{C}_\bullet^< ( \Delta , M))_{i+n} \neq 0$. Let $z \in \cat{C}_i^< (\Delta , M)$ be a cycle that is not a boundary; without loss of generality, assume $z$ is multihomogeneous. The complex $\cat{C}_\bullet^< (M)$ is exact, whence $z = d(y)$ for some $y \in \cat{C}_{i+1}^< (M)$. By multihomogeneity, $y = \lambda g^{*(\alpha)} \otimes f_\sigma$ for some $\lambda \in k^\times$ with $|\sigma|=n+i$, $|\alpha|=i$. The assumption that $z$ is not a boundary implies that $\sigma \notin \Delta$, since otherwise $y \in \cat{C}_{i+1} (\Delta, M)$. By definition of the differential of $\cat{C}_\bullet^< (M)$,
$$z = \lambda \cdot \sum_{\{\ell \mid \alpha_\ell >0\}} \sum_{j} (-1)^{j + 1} \chi ((\ell,\sigma_j) \in \I_< (\alpha , \sigma)) x_{\ell \sigma_j} g^{*(\alpha - \epsilon_\ell)} \otimes f_{\sigma \backslash \sigma_j }.$$
Since $z \neq 0$, $(\ell , \sigma_j) \in \I_< (\alpha , \sigma)$ for some $\ell$, $j$. By definition of $\I_< (\alpha , \sigma)$, this means $(\ell , \sigma_k) \in \I_< ( \alpha , \sigma)$ for all $|\alpha_{\leq \ell-1} | \leq j \leq |\alpha_{\leq \ell}|$. This translates to the fact that $\sigma$ is an $\alpha_\ell$-nonface of cardinality $n+i$. Since $\alpha_\ell \geq 1$, the result follows.
\end{proof}

\begin{remark}
The proof of Lemma \ref{lem:linstrandnonfaces} allows one to construct explicit examples of nonzero homology on the complex $\cat{C}_\bullet^< (\Delta , M)$. Let $\clique$ be the simplicial complex associated to the first graph of Example \ref{ex:exampleof1nonface}. Then the element
$$z = x_{22} f_{1,3,4} - x_{23} f_{1,2,4}$$
is a cycle which is not a boundary in $\cat{C}_\bullet^< ( \clique ,M)$. 
\end{remark}

\begin{lemma}\label{lem:1sthomologylemma}
Adopt notation and hypotheses as in Setup \ref{set:linearStrandSetup}. Then the following are equivalent:
\begin{enumerate}
    \item $H_1 ( \cat{C}_\bullet^< (\Delta , M))_{n+1} = 0$,
    \item $\Delta$ has no $1$-nonfaces of cardinality $n+1$.
\end{enumerate}
\end{lemma}

\begin{proof}
The implication $(2) \implies (1)$ is Lemma \ref{lem:linstrandnonfaces}. Conversely, assume that $\sigma \notin \Delta$ is a $1$-nonface of cardinality $n+1$. By definition, there exists some $j$ such that $\sigma \backslash \sigma{j}$ and $\sigma \backslash \sigma_{j+1} \in \Delta$. This means that  $z= (-1)^{j+1} (x_{j\sigma_j} f_{\sigma \backslash \sigma_j} -  x_{j\sigma_{j+1}} f_{\sigma \backslash \sigma_{j+1}})$ is a cycle in $\cat{C}_1^< (\Delta ,M)$ that is not a boundary, since $z = d_2 (g_j^* \otimes f_\sigma )$, and $g_j^* \otimes f_\sigma \notin \cat{C}_2 (\Delta , M)$ by construction.  
\end{proof}


% \ayah{need to fix: hypothesis should be GB-closed; Case 2: take last $i,i+1$ where $i\neq n$ can be removed, show the next can also be removed, contradiction. If $i=n$, follow GB reductions  backwards to get contradiction on being a nonface.}
% \begin{lemma}\label{lem:closedand1nonfaces}
% Let $\Delta$ be a pure $(n-1)$-dimensional simplicial complex on the vertex set $[m]$. If the simplicial complex $\Delta$ is closed, then the associated clique complex $\clique$ has no $1$-nonfaces of cardinality $\geq n+1$.
% \end{lemma}

% \begin{proof}
% Assume that $\clique$ has a $1$-nonface $\sigma \notin \clique$ of cardinality $\geq n+1$. By definition, there exists $j \geq 1$ such that $\sigma \backslash \sigma_j$, $\sigma \backslash \sigma_{j+1} \in \clique$. Let $\Gamma_1 , \dotsc , \Gamma_r$ be the cliques of $\Delta$; then there are two cases:

% Case $1$: $\sigma \backslash \sigma_j$, $\sigma \backslash \sigma_{j+1} \in \Gamma_i$ for some $i$. Since $\Gamma_i$ is a simplex, $|\sigma| = |\Gamma|+1$. Thus there is only $1$ element $\sigma$ not contained in $\Gamma_i$, in which case there are obviously no $1$-nonfaces, since if $\sigma_j \notin \Gamma_i$, then $\sigma \backslash \sigma_{j-1}$ and $\sigma \backslash \sigma_{j+1} \notin \Gamma_i$ (notice that this case is impossible, regardless of closedness).

% Case $2$: $\sigma \backslash \sigma_j \in \Delta_k$, $\sigma \backslash \sigma_{j+1} \in \Gamma_i$ for some $i \neq k$. Without loss of generality, we may assume that $|\sigma| = n+1$ by taking an appropriate subset of $\sigma$. But then $\sigma \backslash \sigma_j \in \Delta_k$, $\sigma \backslash \sigma_{j+1} \in \Delta_i$, and it is clear that all but the $j$th entries of $\sigma \backslash \sigma_j$ and $\sigma \backslash \sigma_{j+1}$ are equal, whence $\Delta$ is not closed.
% \end{proof}

Recall that the standard Eagon-Northcott complex inherits a $\ZZ^n \times \ZZ^m$-grading, as described in Section $3$ of \cite{herzog2015linear}. Since the sparse Eagon-Northcott complexes of Definition \ref{def:gensparseEN} are obtained by simply setting certain entries in the differentials equal to $0$, these maps will remain multigraded in an identical manner. We tacitly use this multigrading for the remainder of this section. 

\begin{theorem}\label{thm:linearstrandforclosedDelta}
Adopt notation and hypotheses as in Setup \ref{set:linearStrandSetup}. Assume that $\Delta$ is an $(n-1)$-pure simplicial complex such that $\clique$ has no $1$-nonfaces of cardinality $n+1$. Let $\inn_<(J_\Delta)$ denote the initial ideal with respect to standard lexicographic order of the determinantal facet ideal associated to $\Delta$. 

Let $F_\bullet$ denote the minimal graded free resolution of $\inn_<(J_\Delta)$; then
$$F_\bullet^\textrm{lin} \cong \cat{C}_\bullet^< (\clique, M).$$
\end{theorem}

\begin{proof}
Let $Z^\textrm{lin} := (\ker d_1)_{n+1}$, where $d_1$ is the first differential of the complex $\cat{C}_\bullet^< (\clique , M)$. By construction, $\cat{C}_1^< (\clique , M)$ is generated in degree $n+1$ and hence induces a homogeneous map
$$\partial : \cat{C}_1^< ( \clique , M) \to Z^\textrm{lin}.$$
Let $0 \neq z \in Z^{\textrm{lin}}$ be an element of multidegree $(\epsilon_s + 1,\epsilon_{i_1}+\cdots + \epsilon_{i_{n+1}})$ (where $1$ denotes the appropriately sized vector of all $1$'s). Set $\tau := \{ i_1 < \cdots < i_{n+1} \}$; by multihomogeneity, there are constants $\lambda_k \in k$ such that
$$z = \sum_{k=1}^{n+1} \lambda_k x_{s i_k} f_{\tau \backslash i_k}.$$
Since $z$ is a cycle of $\cat{C}_1^< (M)$ (where $\cat{C}_\bullet^< (M) := E_\bullet'$ is as in Definition \ref{def:gensparseEN}), there exists $y \in \cat{C}_2^< (M)$ such that $d_2(y) = z$. By multihomogeneity, $y = \lambda g_s \otimes f_\tau$ for some constant $\lambda$, whence $z = \lambda (-1)^{s+1} (x_{s\sigma_s} f_{\sigma \backslash \sigma_s} - x_{s\sigma_{s+1}} f_{\sigma \backslash \sigma_{s+1}} )$. This implies that $\sigma \in \clique$, since otherwise $\clique$ would have a $1$-nonface of cardinality $n+1$, contradicting our assumptions. Thus $Z^\textrm{lin}$ is generated by
$$\{r_s (\sigma) := (-1)^{s+1} (x_{s\sigma_s} f_{\sigma \backslash \sigma_s} - x_{s\sigma_{s+1}} f_{\sigma \backslash \sigma_{s+1}} ) \mid 1 \leq s \leq n, \ \sigma \in \clique, \ |\sigma| = n+1 \}.$$
Moreover, since $\textrm{mdeg} (r_s(\sigma)) \neq \textrm{mdeg} (r_{s'} (\sigma')$ for $s\neq s'$ or $\sigma \neq \sigma'$, the above is a basis. Finally, $d_2 (g_s^* \otimes f_\sigma ) = r_s (\sigma)$, whence the induced map $\partial$ is an isomorphism of vector spaces.
\end{proof}

\begin{remark}
Let $\Delta$ be an $(n-1)$-pure closed simplicial complex. Then $\clique$ has no minimal nonfaces in cardinality $\geq n+1$, since any minimal nonface is in particular a $1$-nonface. This means that $\clique$ satisfies the hypotheses of Theorem $3.1$ of \cite{herzog2015linear}. 
\end{remark}

\begin{theorem}\label{thm:mainpunchline}
Adopt notation and hypotheses as in Setup \ref{set:linearStrandSetup}. Assume that $\Delta$ is an $(n-1)$-pure simplicial complex with no $1$-nonfaces of cardinality $n+1$. Then for all $i \geq 1$,
$$\beta_{i,n+i} (J_\Delta) = \beta_{i,n+i} (\inn_< (J_\Delta)).$$
\end{theorem}

\begin{proof}
Notice that the linear strand of $J_\Delta$ is $\cat{C}_\bullet (\clique , M)$ where $\cat{C}_\bullet$ is the generalized Eagon-Northcott complex of \cite{herzog2015linear}. Then, $\cat{C}_\bullet$ and $\cat{C}_\bullet^<$ have the same underlying free modules, so the result follows.
\end{proof}

\begin{prop}\label{prop: no1nonface} Let $\Delta$ be pure $(n-1)$-dimensional simplicial complex on $m$ vertices, and let $J_\Delta$ be its associated $n$-determinantal facet ideal. If $J_\Delta$ is lcm-closed, then there are no $1$-nonfaces in $\clique$.
\end{prop}

\begin{proof}
It suffices to show that there are no $1$-nonfaces of cardinality $n+1$ in $\clique$. Suppose, seeking contradiction, that $\ff = \{f_1 < \dots < f_{n+1}\}$ is a $1$-nonface of cardinality $n+1$ in $\clique$. By definition, there exists some $f_i$ such that $\aa = \{f_1,\dots, \widehat{f_i}, f_{i+1}, \dots, f_{n+1}\}$ and $\bb = \{f_1,\dots, f_i, \widehat{f_{i+1}},\dots, f_{n+1}\}$ are facets of $\Delta$. Let $\Delta_\aa$ and $\Delta_\bb$ be maximal cliques of $\Delta$ containing $\aa$ and $\bb$, respectively, with nontrivial intersection.
By assumption, $\Delta_\aa\neq \Delta_\bb$. Because $J_\Delta$ is lcm-closed, there exists some facet $\cc\in \Delta_\aa\cap \Delta_\bb$ such that $\LT[\cc]$ divides
$$\textrm{LCM}(\LT[\aa],\LT[\bb]) = x_{1 f_1} x_{2 f_2} \dots x_{i f_i} x_{i f_{i+1}} x_{i+1 f_{i+2}} \dots x_{n,f_{n+1}}.$$
The only possible facets $\cc$ of $\Delta$ satisfying this property are $\aa$ and $\bb$ themselves, so they must be in the same maximal clique of $\Delta$ and $\ff$ is indeed a face in $\clique$, giving the desired contradiction.
\end{proof}

\begin{prop}\label{prop:strandforclosed}
Adopt notation and hypotheses as in Setup \ref{set:linearStrandSetup}. Assume that $\Delta$ is an $(n-1)$-pure lcm-closed simplicial complex. Let $\inn_<(J_\Delta)$ denote the initial ideal with respect to standard lexicographic order of the $n$-determinantal facet ideal associated to $\Delta$. 

Let $F_\bullet$ denote the minimal graded free resolution of $\inn_<(J_\Delta)$; then
$$F_\bullet^\textrm{lin} \cong \cat{C}_\bullet^< (\clique, M).$$
\end{prop}

The proof is an immediate consequence of the following Lemma, proved in \cite{vdb2020maxlideal}.

\begin{lemma}[\cite{vdb2020maxlideal}]\label{lem:easymodelinearstrands}
Let $R$ be a standard graded polynomial ring over a field $k$. Let $G_\bullet$ be a finite linear subcomplex of an acyclic minimal homogeneous complex of free $R$-modules with initial degree $n$, and assume that for all $i\geq 1 $, $\rank (G_i)_{i+n} = \beta_{i,i+n} (H_0 (G_\bullet)).$ 

Let $F_\bullet$ denote a homogeneous minimal free resolution of $H_0 (G_\bullet)$ and assume that for all $i\geq 1$, the map $(d_i)_{i+n} : (G_i)_{i+n} \to (G_{i-1})_{i+n}$ is left invertible. Then $G_\bullet \cong F^{\textrm{lin}}_\bullet$, where $F^{\textrm{lin}}_\bullet$ denotes the linear strand of $F_\bullet$.
\end{lemma}

\begin{remark}
It is important to notice that the condition on $1$-nonfaces is not sufficient for the minimal generators to form a Gr\"obner basis, and is hence more general than the property of being lcm-closed. For example, let $\Delta$ be the simplicial complex with facets ${1,2,3}$, ${1,4,5}$, and ${1,6,7}$. One can verify directly that there are no $1$-nonfaces of cardinality $4$, but calculations in Macaulay2 show that the minimal generating set of the associated determinantal facet ideal does \emph{not} form a Gr\"obner basis.
\end{remark}


==> sections/bettiNumbers.tex <==
\section{Initial Ideals of Interval Determinantal Facet Ideals}

% \begin{setup}\label{set: initialInterval} Let $\Delta$ be an $(n-1)$-dimensional simplicial complex on $m$ vertices such that $J_\Delta$ is an interval determinantal facet ideal. Denote by $\inn(J_\Delta)$ the initial ideal of $J_\Delta$ with respect to $>$ as in Setup \ref{set: leadTerms}.
% \end{setup}

The goal of this section is to study the graded Betti numbers of initial ideals of interval determinantal facet ideals using the lcm-lattice. We begin by recalling some definitions and tools from poset topology. For further reference, see \cite{wachs2006poset}.

\begin{definition}\label{def: properPart} Let $P$ be a poset such that $\abs{P}>1$ with unique top element $\hat 1$ and unique bottom element $\hat 0$. The \emph{proper part} of $P$ is $\overline P\coloneqq P\setminus \{\hat 0, \hat 1\}$.
\end{definition}

\begin{definition}\label{def: lattice} Let $P$ be a poset and let $x,y\in P$. An \emph{upper bound} of $x,y$ is an element $z\in P$ such that $z\geq x$ and $z\geq y$. If $x$ and $y$ have a unique least upper bound, it is called the \emph{join} of $x$ and $y$ and is denoted $x\vee y$. By duality, the \emph{meet} of $x$ and $y$, denoted $x\wedge y$, is defined to be the unique greatest lower bound of $x$ and $y$, if it is exists. If every pair of elements in $P$ has a join and a meet, then $P$ is said to be a \emph{lattice}.
\end{definition}

\begin{definition}\label{def: orderComplex} Let $P$ be a poset. Then the \emph{order complex} of $P$, denoted $O(P)$, is the abstract simplicial complex whose vertices are the elements of $P$ and whose faces are the chains in the poset.
\end{definition}

\begin{remark}\label{rem: homologyPosets} The (co)homology of a poset is understood to mean the reduced simplicial (co)homology of its associated order complex.
\end{remark}

\begin{definition}\label{def: cartProduct} Let $P$ be a $G$-poset and let $Q$ be an $H$-poset. The \emph{cartesian product} (or \emph{direct product}) of $P$ and $Q$ is the $G\times H$-poset $P\times Q$ such that $(x,y)\leq_{P\times Q} (x',y')$ if $x\leq_P x'$ and $y\leq_Q y'$.
\end{definition}

The following theorem gives a poset version of the K\"unneth theorem of algebraic topology.

\begin{theorem}[\cite{wachs2006poset}]\label{thm: homologyCartesianProducts} 
Let $P$ be a $G$-poset and let $Q$ be an $H$-poset. Then for all $r$,
$$
H_r(P\times Q) \cong_{G\times H} \bigoplus_i H_i(P)\otimes H_{r-i}(Q).
$$
If $P$ has a bottom element $\hat 0_P$ and $Q$ has a bottom element $\hat 0_Q$, then for all $r$,
$$
\tilde H_r(P\times Q \setminus \{(\hat 0_P, \hat 0_Q)\} \cong_{G\times H} \bigoplus_i \tilde H_i(P\setminus \{\hat 0_P\})\otimes \tilde H_{r-i-1}(Q\setminus \{\hat 0_Q\}).
$$
If $P$ and $Q$ also have top elements, then for all $r$,
$$
\tilde H_r(\overline{P\times Q})\cong_{G\times H} \bigoplus_i \tilde H_i(\overline P)\otimes \tilde H_{r-i-2}(\overline Q).
$$
\end{theorem}

\begin{definition}\label{def: booleanPoset} Let $Y$ be a set on $n$ elements. Then \emph{Boolean lattice} $B(Y)$ is a poset on the set of subsets of $Y$ with the partial order defined by conclusion.
\end{definition}

\begin{lemma}\label{lem: booleanSphere} If $B(Y)$ is the Boolean lattice on the set $Y$, then $O(\overline{B(Y)}) \cong \S^{\abs{Y}-2}$ and $O(B(Y)\setminus \emptyset) \cong \BB^{\abs{Y}-1}$.
\end{lemma}

\begin{proof}
Observe that $O(\overline{B(Y)})$ is the barycentric subdivision of the boundary of the $(\abs{Y}-1)$-simplex, so it is is homotopy equivalent to an $\S^{\abs{Y}-2}$ sphere. The unique top element of $B(Y)$ cones over the $\overline{B(Y)}$, giving that $O(B(Y)\setminus \emptyset) \cong \BB^{\abs{Y}-1}$.
\end{proof}

The main tool of this section will be the lcm-lattice. The interested reader may consult \cite{GPWlcm} or \cite[Section 58]{peeva2010graded} for more details.

\begin{construction}\label{const: lcmLattice} Let $M = (m_1,\dots, m_r)$ be a monomial ideal in the polynomial ring $S = k[x_1,\dots, x_n]$. Denote by $L_M$ the lattice with elements the least common multiples of subsets of $m_1, \dots, m_r$ ordered by divisibility. The atoms in $L_M$ are $m_1,\dots, m_r$, the top element is $m_M = \lcm(m_1,\dots, m_r)$, and the bottom element is $1$ regarded as the lcm of the empty set. The least common multiple of elements in $L_M$ is their join. The lattice $L_M$ is called the \emph{lcm-lattice} of the monomial ideal $M$.
\end{construction}

\begin{notation}\label{not: openInterval} For $m\in L_M$, denote by $(1,m)_{L_M}$ the open interval in $L_M$ below $m$; it consists of all non-unit monomials in $L_M$ that strictly divide $m$. 
\end{notation}

\begin{theorem}[\cite{GPWlcm}]\label{thm: lcmBettis} Let $M$ be a monomial ideal in a polynomial ring $S$ over a field $k$. Then for $i\geq 1$,
\begin{align*}
    \beta_{i,m}^S(S/M) = \left\{
    \begin{array}{ll}
        \dim \tilde H_{i-2}((1,m)_{L_M};k) & \text{if } 1\neq m\in L_M\\
        0 & \text{if } m\notin L_M.
    \end{array}
    \right.
\end{align*}
\end{theorem}

The first step toward understanding the structure of the lcm-lattice for initial ideals of interval determinantal ideals is to make sense of the structure of the lcm-lattice in the case of only one maximal clique, i.e., the initial ideal of an ideal of maximal minors of a generic matrix.

\begin{notation}\label{not: niceMonomials}
Let $\Xv_i = \{x_{i1},\ldots, x_{im}\}$ for all $1\leq i\leq n$, and let $R = k[\Xv_1,\ldots,\Xv_n]$ be a polynomial ring in the variables of the $\Xv_i$ over a field $k$. Given a monomial $m\in R$, define $X_i(m) \coloneqq \{x_{ij}\in \Xv_i \mid x_{ij}\text{ divides } m\}$ for all $1\leq i\leq n$.

Let $\Delta$ be an $(n-1)$-dimensional simplicial complex, and let $J_\Delta$ be its associated determinantal facet ideal in $R$. Let $\cA$ be a set of pairs $(i,\tau_j)$ such that $\tau = \{\tau_1, \ldots, \tau_k\} \in \clique$ and $k\geq n$. Associate to $\cA$ a monomial $\mm_\cA$ where
$$
\mm_\cA = \prod_{(i,\tau_j)\in\cA} x_{i,\tau_j}.
$$
Similarly, for any square-free monomial $\mm\in R$, denote by $\cA(\mm)$ the set of pairs $(i,j)$ that divides $\mm$. Endow $\cA(\mm)$ with the ordering $(i_1, j_1)<(i_2, j_2)$ when $i_1 < i_2$ or when $i_1 = i_2$ and $j_1 < j_2$.
% Denote by $\cA(\mm)_2$ the ordered set $\{j_1, j_2, \ldots, j_k\}$ where $(i_{j_1}, j_1) < (i_{j_2}, j_2) < \dots < (i_{j_k}, j_k)$ and $k = \abs{\cA(\mm)}$.

Let $\aa = (a_1 , \dotsc , a_n)\in\ZZ^n$. Define $\abs{\aa} \coloneqq \sum_{i=1}^n a_i.$, and
$$\aa_{\leq i } := (a_1 , \dotsc , a_i ),$$
where $\aa_{\leq i} = \varnothing$ if $i \leq 0$ and $\aa_{\leq i } = \aa$ if $i \geq n$.

Define the set $\cA(\aa; \tau) = \{(i,\tau_j) \mid i\in [n], \ |\aa_{\leq i-1}| < j \leq |\aa_{\leq i}| \}$, where $\tau$ is a $(k-1)$-face of $\clique$ with $k\geq n$, and $\aa = (a_1,\ldots,a_n)\in \NN^n$, $\abs{\aa} = k$. Set $\mm_k(\aa;\tau) \coloneqq \mm_{\cA(\aa;\tau)}$.
\end{notation}

\begin{example}\label{ex: pairNotation}
Let $\Delta$ be the $2$-dimensional simplicial complex with maximal clique decomposition $\{1,2,3,4\}\cup\{2,3,4,5\}$, so $J_\Delta$ is generated by the maximal minors of a generic $3\times 5$ matrix that are contained in the submatrices given by the first four columns and the last four columns. If $\sigma = \{1,2,3,4\}$ and $\aa = (1,2,1)$, then $m_4(\aa;\sigma) = x_{1,1} x_{2,2} x_{2,3} x_{3,4}$.
\end{example}

\begin{setup}\label{set: lcmDFI} Let $\Xv_i = \{x_{i1},\ldots, x_{im}\}$ for all $1\leq i\leq n$, and let $R = k[\Xv_1,\ldots,\Xv_n]$ be a polynomial ring in the variables of the $\Xv_i$ over a field $k$. Let $\Delta$ be an $(n-1)$-dimensional simplicial complex on $m$ vertices with clique decomposition $\Delta = \bigcup_{i=1}^r \Delta_i$, and let $J_\Delta$ be the determinantal facet ideal associated to $\Delta$. Let $I = \LT(J_\Delta)$ as in \ayah{add reference to definition of LT}, and let $L_I$ denote the lcm-lattice of $I$.
\end{setup}

\begin{prop}\label{prop: linStrandBettis} Adopt notation and hypotheses of Setup \ref{set: lcmDFI}. If $m = \mm_k(\aa;\tau)$ for some $\aa\in\NN^n$ and $\tau\in\clique$ with $k\geq n$, then

\begin{align*}
    \beta_{i,m}(R/I)) = \left\{
    \begin{array}{ll}
        1 & \text{if } i = k-n+1\\
        0 & \text{otherwise}.
    \end{array}
    \right.
\end{align*}
Moreover, for any other monomial $w$ such that every $x_{ij}$ dividing $w$ divides a generator coming from a single clique of $\Delta$ but is not of the form $\mm_k(\aa;\tau)$, $\beta_{i,w}(R/I) = 0$ for all $i$.
\end{prop}

\begin{proof}
Let $B_i = B(X_i(m))\setminus \hat 0_{B(X_i(m))}$, and let $m_i=\abs{X_i(m)}$. Then each $B_i$ is isomorphic to a simplicial ball $\BB^{\abs{m_i}-1}$ by Lemma \ref{lem: booleanSphere}, and
$$
(1,m)_{L_I} \cong (B_1\times B_2\times \dots \times B_n)\setminus \{m\}.
$$
The Cartesian product of simplicial balls is a simplicial ball, since $\BB^i\times \BB^j \cong \BB^{i+j}$, so $(1,m)_{L_I} \cong \S^{k-n-1}$. Applying Theorem \ref{thm: lcmBettis} gives the desired result.

Now, consider some monomial $w$ that cannot be written as $\mm_k(\aa;\tau)$. If it is not squarefree or divisible by at least one variable from each color class $\Xv_i$, then it does not appear in the lcm-lattice and $\beta_{i,w}(S/I)=0$ for all $i$ by Theorem \ref{thm: lcmBettis}.

Assume that $w$ is squarefree and is divisble by at least one variable from each color class $\Xv_i$, and that it is divisible by a squarefree monomial $a = x_{i_1 j_1}\cdots x_{i_k j_k}$ such that $i_1\leq \dots \leq i_k$ and $j_1\geq \dots \geq j_k$. Assume that for each $x_{i_\ell j_\ell}$ dividing $a$, some generator of $I$ dividing $2$ contains it. Proceed by double induction on $\abs{w}$ and $\abs{a}$. First assume that $a = x_{i_1 j_1} x_{i_2 j_2}$ where $i_1<i_2$ and $j_1\geq j_2$ and $\abs{w} = n+2$, where $\abs{X_{i_1}(m)} = \abs{X_{i_2}(m)} = 2$ and $\abs{X_i(m)} = 1$ for all other $i$. Then $w$ covers the monomials $m_1 = \frac{w}{x_{i_1 j_1}}$ and $m_2 = \frac{w}{x_{i_2 j_2}}$ in the lcm-lattice $L_I$. By assumption, $m_1$ and $m_2$ can both be written in the form $\mm_k(\aa,\tau)$ for some $\aa,\tau$, so $(1, m_1]\cong (1,m_2] \cong \B^1$, and they intersect at the generator $m_3 = \frac{w}{a}$. Therefore, $O(1,m_1]$ and $O(1,m_2]$ form a simplicial cover for $O(1,w)$ and have contractible intersection; applying the Nerve Lemma \ayah{add, cite}, this implies that $O(1,w)$ is contractible.

\ayah{finish induction}
% Now assume $\abs{a} = 2$ as above but $\abs{w} = n+2+k$, and proceed by induction on $k$. Agai
\end{proof}

\ayah{add example?}



% \begin{theorem}\label{thm: mgBettis} Adopt notation and hypotheses of Setup \ref{set: lcmDFI} and, in addition, let $J_\Delta$ be an interval determinantal facet ideal, so that $I = \LT(J_\Delta) = \inn(J_\Delta)$ by \ayah{add theorem}. Order the cliques of $\Delta$ lexicographically $\Delta_1 < \Delta_2 < \dots < \Delta_r$ where $\Delta_i < \Delta_j$ if $\min(V(\Delta_i))<\min(V(\Delta_j))$. This ordering is well defined because all maximal cliques of $\Delta$ are intervals.

% Let $\ww$ be a product of monomials $\ww_1\cdot\ww_2\dots \ww_\ell$ satisfying the following conditions:
% \begin{enumerate}
%     \item $\ww_i = \mm_{k_i}(\aa^i;\tau^i)$ for some $\aa\in \NN^n$ and some $\tau^i\in \clique$ such that $\abs{\tau^i}\geq n$,
%     \item $\tau^i\cup \tau^j\notin \clique$ for any $i\neq j$, and any clique containing $\tau_i$ is strictly less than any clique containing $\tau_j$,
%     \item for any $x_{jp}\in X_j(\ww_{i_1})$ and any $x_{jq}\in X_j(\ww_{i_2})$ with $i_1 < i_2$, we have that $p<q$. 
% \end{enumerate}
% Then for $i\geq 1$,
% \begin{align*}
% \beta_{i,\ww}(R/I) = \left\{
%     \begin{array}{ll}
%         1 & \text{ if } i = \abs{\ww} - \ell(n-1)\\
%         0 & \text{ otherwise}.
% \end{array}
% \right.
% \end{align*}
% \end{theorem}

% \begin{proof}
% It suffices to show that $\dim \tilde H_i(1,\ww) = 1$ when $i=\abs{\ww}-\ell(n-1)-2$ and is $0$ otherwise, since applying Theorem \ref{thm: lcmBettis} gives the desired result. 

% $$
% [1,\ww]_{L_I} = [1,\ww_1]_{L_I} \times \dots \times [1,\ww_\ell]_{L_I}.
% $$
% Proceed by induction on $\ell$. The case $\ell=1$ follows from Proposition \ref{prop: linStrandBettis}. Apply the induction hypothesis and assume that the theorem holds for a product of $\ell-1$ monomials satisfying conditions (1)-(3) of the the theorem statement. Applying Theorem \ref{thm: homologyCartesianProducts} and the above observation,
% \begin{align*}
% \tilde H_r(1,\ww_1\dots\ww_\ell)_{L_I} &\cong \bigoplus_i \tilde H_i(1,\ww_1\dots\ww_{\ell-1})_{L_I} \otimes \tilde H_{r-i-2}(1,\ww_\ell)_{L_I}\\
% &\cong \tilde H_{\abs{\ww_1\dots \ww_{\ell-1}} - (\ell-1)(n-1)-2}(1,\ww_1\dots\ww_{\ell-1})_{L_I} \otimes \tilde H_{k_\ell - n -1}(1,\ww_\ell)_{L_I}
% \end{align*}
% and is $0$ otherwise. So $\dim \tilde H_r (1,\ww)_{L_I}$ is only nonzero when $r = \abs{\ww}-\ell(n-1)-2$, as desired.
% \end{proof}

% \ayah{add example?}

% \begin{theorem}\label{thm: homology0} For any monomial $m$ that cannot be written as a product of monomials satisfying conditions (1)-(3) in the statement of Theorem \ref{thm: mgBettis}, $\beta_{i,m}(R/I) = 0$ for all $i$.
% \end{theorem}

% \begin{proof}
% If $m$ cannot be written as a product of monomials satisfying conditions (1)-(3) in the statement of Theorem \ref{thm: mgBettis}, then it is
% \begin{enumerate}
%     \item[(a)] $m$ is not squarefree.
%     \item[(b)] $m$ is not divisible by at least one variable from each $\Xv_i$.
%     \item[(c)] Every $x_{ij}$ dividing $m$ is in the same clique, but $m$ is divisible by some squarefree monomial $x_{i_1 j_1} \cdots x_{i_k j_k}$ where $i_1\leq \dots \i_k$ but $j_1\geq \dots j_k$.
%     \item[(d)] $m$ is divisible by 
% \end{enumerate}
% \end{proof}

% \ayah{some exposition}

% \begin{cor}\label{cor: linearStrandDFI} Adopt notation and hypotheses as in \ayah{add}. Then
% $$
% \beta_{i,i+\ell}(R/\inn(J_\Delta)) = \beta_{i,i+\ell}(R/J_\Delta) = \binom{\ell-i+1}{\ell-1} f_{\ell+i-1}(\clique)
% $$
% where $f(\clique)$ is the $f$-vector of $\clique$. In particular, the Betti numbers in the linear strand of $J_\Delta$ and $\inn(J_\Delta)$ coincide.
% \end{cor}

% \begin{cor}\label{cor: pdim} \ayah{fix setup and notation} Adopt notation and hypotheses as in ... Then
% \begin{enumerate}
%     \item $\reg(R/J_\Delta) = \max \{ \abs{\cH} \mid \cH \text{ is a clique disjoint set of facets of } \Delta\}\cdot (n-1)$.
%     \item Set $p = \max\{\sum_{f\in\cS} \abs{f} \mid \cS \text{ is a clique disjoint set of faces of } \clique \}$. Then $\pdim(R/J_\Delta) = p - \reg(R/J_\Delta)$.
% \end{enumerate}
% \end{cor}

% \ayah{add proof}

% The following result is an application of Theorems \ref{thm: mgBettis} and \ref{thm: homology0}.

% \begin{theorem}\label{thm: consecutiveCancellations} Let $\Delta$ be a pure $(n-1)$-dimensional simplicial complex which is closed. 
% \begin{itemize}
% \item If $n=2$ (so $\Delta$ coincides with a graph $G$) and $\reg(S/J_G) \leq 3$, then $\beta_{i,j}(R/J_G) = \beta_{i,j}(R/\inn(J_G))$ for all $i,j$. In particular, if $G$ has at most two maximal cliques, the standard graded betti numbers of $\inn(J_G)$ and $J_G$ coincide.
% \item When $n>2$, the standard graded Betti numbers of $R/J_\Delta$ and $R/\inn(J_\Delta)$ coincide.
% \end{itemize}
% \end{theorem}

% Before proving the theorem above, recall the following definition.

% \begin{definition}[\cite{peeva2010graded}]\label{def: consecCancel} A sequence $q_{i,j}$ of numbers is obtained from a sequence $p_{i,j}$ by a \emph{consecutive cancellation} if there exist indexes $s$ and $r$ such that

% \begin{align*}
% q_{s,r} = p_{s,r} - 1, \qquad q_{s+1,r} = p_{s+1,r} -1,\\
% q_{i,j} = p_{i,j} \qquad \text{for all other values of } i,j.
% \end{align*}
% \end{definition}

% \begin{proof}[Proof of Theorem \ref{thm: consecutiveCancellations}]
% Observe that the Betti numbers of $R/J_\Delta$ can be obtained from the Betti numbers of $R/\inn(J_\Delta)$ by consecutive cancellations (see \cite[Theorem 22.12]{peeva2010graded}). By Theorem \ref{thm: MGbettis}, the basis elements of the modules in the free resolution of $S/\inn(J_\Delta)$ are given by monomials of the form

% $$
% \mm_{k_1}(\aa^1, \tau^1) \cdots \mm_{k_\ell}(\aa^\ell, \tau^\ell)
% $$
% which have homological degree $\sum k_i - \ell(n-1)$ and internal degree $\sum k_i$. 

% A consecutive cancellation is only possible when both $\beta_{i,j}(R/\inn(J_\Delta))$ and $\beta_{i+1,j}(R/\inn(J_\Delta))$ are nonzero. Assume that $\beta_{i,j}(R/\inn(J_\Delta))$ is nonzero. Then it has basis elements above where $j = \sum k_i$ and $i = \sum k_i - \ell(n-1) = j-\ell(n-1)$; that is, $j-i = \ell(n-1)$. However, if $\beta_{i+1,j}(R/\inn(J_\Delta))$ is also nonzero, then $j-i-1$ must also be divisible by $n-1$. Since two consecutive numbers cannot be divisible by $n-1$ unless $n=2$, $\beta_{i+1,j}(R/\inn(J_\Delta))=0$ and no consecutive cancellations are possible. Therefore, the Betti numbers of $R/J_\Delta$ and $R/\inn(J_\Delta)$ coincide for $n>2$.

% In the case when $n=2$ and $\reg(\inn(J_G))\leq 3$, observe that by Corollary \ref{cor: linearStrandDFI}, the standard graded Betti numbers in the first linear strand of $J_G$ and $\inn(J_G)$ coincide \ayah{cite EN paper}. Therefore, no consecutive cancellations are possible between the first row and the second row of the Betti table of $\inn(J_G)$.
% \end{proof}

% \begin{remark} \ayah{fix this} Consecutive cancellations may still be possible more generally in the case when $n=2$. However, Ene, Herzog, and Hibi conjectured in \cite{EHH2011-CMBEIs} that when $n=2$, the Betti numbers of $J_\Delta$ and $\inn(J_\Delta)$ coincide whenever the minimal generating set of $J_\Delta$ forms a Gr\"obner basis with respect to $<$; this is the case when $J_\Delta$ corresponds to a closed binomial edge ideal. By Corollary \ref{cor: linearStrandDFI}, the linear strand of a closed binomial edge ideal always coincides with that of its initial ideal. Similarly, by a result of Conca and Varbaro in \cite{CV20-sqfree}, all extremal Betti numbers of the $J_\Delta$ and $\inn(J_\Delta)$ coincide.
% \end{remark}
